Systematic Evaluation and User Study of Privacy of Default Apps in Apple's Mobile Ecosystem

Users need to configure default apps when they first start using their devices. The privacy configurations of the default apps do not always match what users think they have initially enabled. We first systematically evaluated the privacy configurations of default apps. We discovered serious issues with the documentation of the default apps. Based on these findings, we explored users' experiences with an interview study (N=15). Our findings from both studies show that: the instructions of setting privacy configurations of default apps are vague and lack required steps; users were unable to disable default apps from accessing their personal information; users assumed they were being tracked by some default apps; default apps may cause tensions in family relationships because of information sharing. Our results illuminate on the privacy and security implications of configuring the privacy of default apps and how users perceive and understand the mobile ecosystem.

==> InterviewGuide.tex <==
You have been invited to participate in a research study. Participation in this study is voluntary. You can discontinue your participation in the study at any time. Should you discontinue your participation, you will not be subject to any negative consequences. The interview is divided into two parts: General questions and Practical tasks. You may use your personal devices for the practical tasks. Please feel free to ask during the interview process and enquire about the questions.

(Participants signed a consent form before proceeding to the interviews, read information sheet about the study and the privacy policy for handling data)

\subsubsection{General Questions:}
\begin{enumerate}
    \item What is the model of your iPhone?
    \item What is the model of your Macbook?
    \item Do you have an iCloud Account?
    \item Do you have an Apple ID?
    \item Did you set up your iPhone by yourself?
    \item Did someone else help you setup your iPhone?
    \item Did you setup your MacBook by yourself?
    \item Did someone else help you setup your MacBook?
    \item How was the setup for you? [Follow up question: What did you think of the instructions that were provided to guide you? Did you notice any instructions about collecting your personal information?]
    \item Are you using TouchID?
    \item Where do you think your fingerprint information is stored? For instance, on the drive or on the Cloud? {Follow up question: Do you remember reading anything about this when setting up your fingerprint? How do you wish that you were informed?}
    \item What apps that were already on your iPhone were you using? [Follow up question: Do you think they are useful?]
    \item What apps that were already on your MacBook were you using? [Follow up question: Do you think they are useful?]
    \item Are you using FindMy on your iPhone?
    \item Are you using FindMy on your MacBook?
    \item Do you know what FindMy is used for? [Follow up question: Have you ever been in a situation where you had to use FindMy? How was that experience? Do you think FindMy can be improved to be more effective?]
    \item Do you know what is Siri?
    \item Do you know what Siri is used for?
    \item If you use Siri, how does Siri help you? [Follow up question: Do you know the type of information Siri collects?]
    \item Does Siri collect your voice recordings? [follow up question: Do you think Siri is collecting more that it needs?]
    \item Are you okay with Siri collecting your voice recordings? [Follow up question: How do you think Siri can be improved to not collect so much?]
    \item Do you use Location Services on your iPhone? 
    \item Do you use Location Services on your MacBook?
    \item Does your iPhone store the place that you have visited? [Follow up questions: Is it always enabled? What do you think about a device knowing your whereabouts?]
    \item Would you be okay with your location being stored? [Follow up questions: What situations do you think this can prove to be useful the most?]
    \item Do you know which applications collect your location data? [Follow up questions: Is it easy to find?]
    \item Do you know what Apple Analytics are?
    \item Do you think apple collects your personal information? [Follow up questions: Is there some information that you don’t want to be collected? Do you know how to stop apple from collecting that information? How do you wish you were informed about not sharing some data? How would you want to see this option?]
    \item What kind of information do you think Apple Collects?
    \item Do you store your pictures, videos on your phone? [Follow up questions: Do the photos and videos that you store contain sensitive information? Do you use any techniques to protect these photos and videos?]
    \item Do you know that Apple has access to the information you store on the Cloud such as your Photos, videos etc.? 
    \item Apple claims that it collects your personal information to improve your experience. What are your thoughts about this? 
    \item Can you stop data sharing? [Follow up questions: Do you think Apple makes it clear on how to stop data sharing? How do you think that can be improved?]
    \item Is your data stored anywhere else other than your phone? [Follow up questions: This could be the Cloud or on your Phone?]
    \item What happens to your data once you stop sharing it with Apple? [Follow up questions: Do you think there are other ways to let you know about the fate of your data? Do you remember reading this anywhere? Do you think users should be compensated for their data?]
    \item Do you use iMessage?
    \item Do you use Facetime?
    \item Are you aware that iMessage and Facetime delete your messages and calls after some time? [Follow up questions: Do you know that you can control the time your messages and calls are stored?]
    \item Do you use family sharing?
    \item Do you use Family sharing feature on your iPhone? 
    \item Do you use Family sharing feature on your MacBook?
    \item If so, how many family members have access to the Family Shared devices?
    \item Do you have the Public Sharing feature in Family sharing enabled?
    \item Do you know that the family members using the Family feature can see your purchases, location etc.?
    \item Do you share your location on the devices that have the Family Sharing feature?
    \item Do you use Safari on your iPhone?
    \item Do you use Safari on your MacBook? 
    \item Do you share your browsing information across your devices on your iPhone?
    \item Do you share your browsing information across your devices on your MacBook? [Follow-up question: How does that affect your experience?]
    \item Do you know what information Safari shares across your devices?
    \item Are you okay with Safari sharing information about your browsing across devices?

\end{enumerate}

\subsubsection{Practical Questions}
These questions should be performed on both the iPhone and the MacBook.
\begin{enumerate}
    \item Do you know how to disable Safari from sharing your information between devices on your iPhone?
    \item Do you know how to disable Safari from sharing your information between devices on your MacBook? [Follow up questions: Can you talk about your feelings after completing this process?]
    \item What do you think happened now that you have disabled sharing? [Follow up questions: How do you think this can be communicated to you in a better way?]
    \item Do you think that turning off sharing in Safari across the devices guarantees that no data is shared anymore across these devices? [Follow up questions: How do you think this can be communicated to you in a better way? Do you think the current terms and conditions statement can be improved?]
    \item Do you know how to delete history/bookmarks and other information from Safari on your iPhone?
    \item Do you know how to delete history/bookmarks and other information from Safari on your MacBook? [Follow up questions: Can you talk about your feelings after completing this process?]
    \item What do you think happened now that you have deleting your stored information?
    \item Do you think your history from your previous search has been deleted? [Follow up questions: Do you think it is Apple’s responsibility to notify users when their data has been completely deleted?]
    \item Do you know how to turn off Apple Pay in Safari on your iPhone?
    \item Do you know how to turn off Apple Pay in Safari on your MacBook?
    \item Apple Pay is turned on by default for Safari. Tell me your thoughts about that?
    \item Do you know that your device may send information such as location, topics of interest, search queriers, suggestions you have selected and related usage data to Apple? 
    \item Do you know how to disable the public sharing in Family Sharing on your iPhone? 
    \item Do you know how to disable the public sharing in Family Sharing on your MacBook?
    \item Do you know how to hide your purchases in Family Sharing on your iPhone?
    \item Do you know how to hide your purchases in Family Sharing on your MacBook?
    \item Do you know how to hide your location in Family Sharing on your iPhone?
    \item Do you know how to hide your location in Family Sharing on your MacBook?
    \item Do you know that if Purchase Sharing is enabled, members of your family will automatically be able to access many of your past and future App Store, Apple Books and Apple Music purchases, unless you choose to hide those purchases? How do you feel about that?
    \item Do you know how to disable iMessage on your iPhone?
    \item Do you know how to disable iMessage on your MacBook?
    \item Do you know how to disable Facetime on your iPhone?
    \item Do you know how to disable Facetime on your Macbook?
    \item Do you know that iMessage and Facetime use end-to-end encryption? 
    \item Do you know what end-to-end encryption means? [Follow up question: Do you know that iMessage and Facetime use end-to-end encryption?]
    \item Do you know that Apple can't read the contents of your conversations when they are in transit between devices? How do you feel about that? 
    \item Do you know that iMessage messages can be set to be deleted after 30 days, a year or stored forever? How do you feel about that? 
    \item Are you okay with apps sharing your information with Siri? 
    \item Do you know how to disable Siri from collecting data from apps on your iPhone?
    \item Do you know how to disable Siri from collecting data from apps on your Macbook?
    \item Do you know how to disable Siri on your iPhone?
    \item Do you know how to disable Siri on your MacBook?
    \item Do you know that the things you say, and dictate will be sent to Apple to process your requests? How do you feel about that?
    \item After six months, your request history is dissociated from the random identifier and may be retained for up to two years to help Apple develop and improve Siri. What do you think about that? 
    \item Do you think your older voice data is deleted once you have disabled Siri?  
    \item Do you know that a small subset of requests that have been reviewed may be kept beyond two years without the random identifiers for ongoing improvement of Siri? 
    \item Do you know that apps contribute information to personalize Siri?  
    \item Do you know how to check which application collects your location data on your iPhone?
    \item Do you know how to check which application collects your location data on your MacBook?
    \item Do you know how to disable Location on your iPhone? 
    \item Do you know how to disable Location on your MacBook? [Follow-up question: What do you think happened?]
    \item Do you know that you can disable the live locations for applications separately? How do you feel about that? Does it make sense? 
    \item Do you think that upon disabling Location services that Apple cannot obtain your location anymore?
    \item Apple doesn’t completely anonymize your data, leaving in things like location. How do you feel about that?
    \item How accurate do you think your location that is collected is?
    \item Your device reminds you from time to time that an application is using your location. How do you feel about that? 
    \item To deliver relevant suggestions, Apple may use the IP address of your internet connection to approximate your location. How do you feel about that? [Follow up question: What are your thoughts?]
\end{enumerate}


==> Participant_list.tex <==
% Table generated by Excel2LaTeX from sheet 'Participant list'
\begin{table*}[!ht]
  \centering
  \caption{Add caption}
    \begin{tabular}{\linewidth}{clllc}
    \toprule
    P\#   & \multicolumn{1}{c}{Occupation} & \multicolumn{1}{c}{iPhone Model} & \multicolumn{1}{c}{Macbook Model} & Default apps \\
    \midrule
    P01   & PhD candidate Computer Science & iPhone 6S & MacBook Pro: 2012+ & 1,4,7,8 \\
    P02   & Software Developer & iPhone X & MacBook: 2015+ & 1- 5,7,8 \\
    P03   & Industrial Engineering researcher & iPhone SE (2016) & MacBook Pro: 2012+ & 4,5,7,8 \\
    P04   & GIS specialist / Msc student in forestry &  iPhone 7 & MacBook Pro: 2012+ & 1-5,7,8 \\
    P05   & Educational Sciences student & iPhone SE (2020) & MacBook Air: 2012+ & 1,2,4,5,8 \\
    P06   & UI/UX Designer, front-end web developer & iPhone 11, Pro, Pro Max & MacBook Pro: 2012+ & 2-8 \\
    P07   & Hospitality Management student &  iPhone 7 & MacBook: 2015+ & 1-4, 6-8 \\
    P08   & Architect &  iPhone 7 & MacBook Pro: 2012+ & 1-5, 7,8 \\
    P09   & Economist & iPhone SE (2016) & MacBook: 2015+ & 1 - 4, 7 \\
    P10   & Assisstant & iPhone 11, Pro, Pro Max & MacBook: 2015+ & 1-5, 7,8 \\
    P11   & Graphic designer & iPhone XR & MacBook Air: 2012+ & 1,2,4,5,7 \\
    P12   & Unemployed & iPhone 11, Pro, Pro Max & MacBook Air: 2012+ & 2 - 5,  \\
    P13   & Program manager & iPhone 11, Pro, Pro Max & MacBook Pro: 2012+ & 1,2,4-8 \\
    P14   & Labratory Technician (Sculptor) & iPhone 11, Pro, Pro Max & MacBook Pro: 2012+ & 1-5, 7,8 \\
    P15   & Document Controller & iPhone 11, Pro, Pro Max & MacBook: 2015+ & 1-8 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Sections/abstract.tex <==
Users need to configure default apps when they first start using their devices.  The privacy configurations of the default apps do not always match what users think they have initially enabled. We first systematically evaluated the privacy configurations of default apps. We discovered serious issues with the documentation of the default apps. Based on these findings, we explored users' experiences with an interview study (N=15). Our findings from both studies show that: the instructions of setting privacy configurations of default apps are vague and lack required steps; users were unable to disable default apps from accessing their personal information; users assumed they were being tracked by some default apps; default apps may cause tensions in family relationships because of information sharing. Our results illuminate on the privacy and security implications of configuring the privacy of default apps and how users perceive and understand the mobile ecosystem.

==> survey.tex <==
This is a screening survey to our research study. Please fill out this survey and we will contact you if you are eligible for the study.

\noindent The actual study is in the form of an interview. The interview will take place over Zoom. Participation in this study will take approximately 1 hour. The session will be voice recorded.
To participate in this survey, please provide us with the following information.

\noindent (Mandatory fields are marked with an asterisk (*) and must be filled in to complete the form.)


1. Do you own both an iPhone and a Macbook? *
\begin{itemize}
    \item  I use both an IPhone and a Macbook
    \item I use an iPhone only
    \item I use a Macbook only
    \item I do not use an iPhone or a Macbook
\end{itemize}

2. Your iPhone Model
\begin{itemize}
    \item iPhone 11, 11 Pro, 11 Pro Max
    \item iPhone XS and XS Max
    \item iPhone XR
    \item iPhone X
    \item iPhone 8
    \item iPhone 8 Plus
    \item iPhone 7
    \item iPhone 7 Plus
    \item iPhone 6S
    \item iPhone 6S Plus
    \item iPhone SE (2020)
    \item iPhone SE (2016)
    \item I do not use an iPhone
\end{itemize}
3. Your iPhone Operating System Version
(To check, go to Settings > General > About > Software Version): \textit{type here operating system version}.
\newline
4. Your Macbook Model
\begin{itemize}
    \item MacBook: 2015 and later
    \item MacBook Air: 2012 and later
    \item MacBook Pro: 2012 and later
    \item I do not use a MacBook
\end{itemize}
5. Your Macbook Operating System Version
(To check, go to the top left apple symbol on your menu bar and select About this Mac): \textit{type here operating system version}.
\newline
6. Do you use the following applications? (Please select all that apply)
\begin{itemize}
    \item TouchID
    \item Find My
    \item Siri
    \item Safari
    \item Location Services
    \item Family Sharing
    \item iMessage
    \item Facetime
\end{itemize}

7. What is your gender (or write "prefer not to say")?

8. Age *
\begin{itemize}
    \item 18 - 29
    \item 30 - 39
    \item 40 - 49
    \item 50 - 59
    \item 60+
\end{itemize}

\noindent 9. Occupation *: \textit{enter occupation here}
\newline
10. Your email address we can use to contact you if you are chosen for the interview *: \textit{enter your email here}


